Efficiently intertwining widening and narrowing

Non-trivial analysis problems require posets with infinite ascending and descending chains. In order to compute reasonably precise post-fixpoints of the resulting systems of equations, Cousot and Cousot have suggested accelerated fixpoint iteration by means of widening and narrowing. The strict separation into phases, however, may unnecessarily give up precision that cannot be recovered later, as over-approximated interim results have to be fully propagated through the equation the system. Additionally, classical two-phased approach is not suitable for equation systems with infinitely many unknowns---where demand driven solving must be used. Construction of an intertwined approach must be able to answer when it is safe to apply narrowing---or when widening must be applied. In general, this is a difficult problem. In case the right-hand sides of equations are monotonic, however, we can always apply narrowing whenever we have reached a post-fixpoint for an equation. The assumption of monotonicity, though, is not met in presence of widening. It is also not met by equation systems corresponding to context-sensitive inter-procedural analysis, possibly combining context-sensitive analysis of local information with flow-insensitive analysis of globals. As a remedy, we present a novel operator that combines a given widening operator with a given narrowing operator. We present adapted versions of round-robin as well as of worklist iteration, local and side-effecting solving algorithms for the combined operator and prove that the resulting solvers always return sound results and are guaranteed to terminate for monotonic systems whenever only finitely many unknowns (constraint variables) are encountered. Practical remedies are proposed for termination in the non-monotonic case.

==> classical.tex <==
%!TEX root = main.tex

\section{Classical Widening/Narrowing Technique}

Constraint systems, as they are used in abstract interpretation, have the form
\begin{align*}
  x_0     &\sqsupseteq F_0(x_0,x_1,\cdots,x_{n-1})\\
          &\;\: \vdots\\
  x_{n-1} &\sqsupseteq F_n(x_0,x_1,\cdots,x_{n-1})
\end{align*}
and are described by functions $F_i: L^n \to L$ over a complete lattice $L$ 
with ordering $\sqsubseteq$.
% 
In the case of abstract interpretation, the variables relate to
control flow points of a program, the values have a semantic interpretation 
about that program, and $\sqsubseteq$ corresponds to the implication order 
in that interpretation. 

The goal is to find values for the variables $x_i$ so that 
all inequations in the constraint system hold. Moreover, smaller solutions,
with respect to the ordering $\sqsubseteq$, are preferred over a larger solution
as they imply a stronger logical property about the program.
%
Solving a constraint system typically consists of applying the function 
$$G^\sqcup_i\;(x_0,\ldots,x_n) = (x_0,\ldots,x_{i-1},x_i\sqcup F_i\:(x_0,\ldots,x_n),x_{i+1},\ldots,x_n)$$
in a sequence, starting with a vector of just bottom values. 
This function updates the $i$-th variable, using the value $x_i\,\sqcup\,F_i\;(x_0,\ldots,x_n)$ and
leaves all other variables with their previously held value.
%
The sequence $k=\left<k_0,k_1,\dots,k_m\right>$, used for calculating a solution vector
$\vec{X} = (G^\sqcup_{k_m}\circ \ldots \circ G^\sqcup_{k_1} \circ G^\sqcup_{k_0})\;(\bot,\ldots,\bot)$
is called the \emph{iteration strategy} as discussed by \citet{Bourdoncle93}.
The job of the solver is to come up with an iteration strategy that leads to a solution.
% cite Bourdoncle
%
%Solving a constraint system typically consists of assigning $\bot$, the least value of $L$, to
%all variables $x_i$ and thereafter changing the values of variables 
%by some amount until all equations are satisfied.

The existence of a unique least solution depends on the properties of 
the functions $F_i$. 
%
One such sufficient condition that guarantees the \emph{existence} 
of the least solution is the requirement for functions $F_i$ to be monotone 
in each of its arguments. 
%
Finding the least solution, though, might still be impossible in finite time even
if the least solution exists. It can be found, however, in the case the function
is monotone and there are no infinite strictly ascending chains in $L$. 

\begin{wrapfigure}{r}{0.44\textwidth}
\vspace{-1.2em}
\begin{lstlisting}[basicstyle=\small,frame=single,mathescape=true,morekeywords={for,do,to}]  
  for i := 0 to $n-1$ 
    x$_i$ := $\bot$;
  do {
    dirty := false;
    for i := 0 to n-1 {
      if x$_i\neq{} $F$_i$($x_0,\ldots,x_{n-1}$) {
        x$_i$ := x$_i$ $\sqcup$ F$_i$($x_0,\ldots,x_{n-1}$);
        dirty := true;
      }
    }
  } while (dirty)
\end{lstlisting}
\vspace{-1em}
\caption{Round-Robin solver}\label{f:rr}
\vspace{-1em}
\end{wrapfigure}
Solving a constraint system where the functions $F_i$ are monotone and where all 
strictly ascending chains in $L$ are finite, can be, for example, done with a Round-Robin 
algorithm in Figure~\ref{f:rr}, that implements an iteration strategy 
$\left<1,2,\ldots,n-1,1,2,\ldots,n-1,\ldots\right>$.
%
%First variables are initialized to $\bot$, then, in a loop, new values are calculated
%from old values by applying a function $F_i$ to the vector of current
%values $(x_0, \ldots,x_{n-1})$. The loop is repeated until all values stabilize.
%
Termination of the algorithm can be concluded from the following observations:
first, the new value for each variable is always bigger or equal to the old value,
second, the value of each variable can increase only a limited number of times,
third, there are exactly $n$ variables.
%
It can be shown that this algorithm not only gives you a solution of the constraint system, 
but produces the least solution.

Note, that the value $x_i := x_i \sqcup F_i(x_0,\ldots,x_{n-1})$ is accumulated in a way
not necessary for monotone functions $F_i$. This accumulation, however, adds to 
the robustness of the algorithm. In case of non-monotone functions,
a particular system might still be solvable using accumulation where the 
straight assignment would not terminate. 


In the case where the functions $F_i$ are monotone, but where the lattice $L$ contains
infinitely long ascending chains, the previous solving algorithm would not necessarily 
terminate. The classical solution, provided by \citet{CousotCousot77}, is to use a special widening
operator $\widen$ for updating the values of variables $x_i$. 
The operator $\widen: L \to L \to L$ is a widening operator if 
  $\forall x, y\in L : x \sqcup y \sqsubseteq x \widen y$,
  and for every chain $x_0\sqsubseteq x_1\sqsubseteq x_2\sqsubseteq \ldots\;$
  the chain $y_0\sqsubseteq y_1\sqsubseteq y_2\sqsubseteq \ldots\;$, where 
  $y_0=x_0$ and $y_{i+1} =y_i\widen x_{i+1}$, is not strictly ascending.
%
To use this operator in the solver we simply replace the least upper bound operation in the accumulation
$x_i = x_i \sqcup F_i(x_0,\ldots,x_{n-1})$ with the widening operator $x_i = x_i \widen F_i(x_0,\ldots,x_{n-1})$.
%
This method of widening has an upside that the algorithm will
definitely terminate even if $L$ contains infinitely long strictly increasing chains but also 
a downside that the result returned might not be the \emph{least} solution.

%In the context of abstract interpretation, intuitively, applying widening loses information.
%We will be looking at two ways to limit the loss of information: first, we can limit the 
%use of widening, and second, one can try to recover some information later. 
%It is not necessary to apply widening for every variable --- actual widening can be 
%limited to $W\subseteq\mathbb{N}^n$ widening points, elsewhere the updated value can be returned as-is. 
%\[
%  x\; \upds_i\, y =\begin{cases}
%    x\widen y, &\text{ if } i\in W\\
%    y,         &\text{ otherwise }
%  \end{cases}
%\]
%Widening is only needed if there exists a feedback loop between variables, more specifically, 
%each feedback loop must contain at least one variable that belongs to $W$. 
%This is safe because stabilization of widening points implies stabilization of all other variables,
%as shown by \citet{Bourdoncle93}.

After getting a non-least solution for a constraint system with monotone functions and
widening operation, one can try to improve the solution by using a narrowing operator $\narrow$.
An operator $\narrow: L \to L \to L$ is a narrowing operator if
  $\forall x, y\in L : y \sqsubseteq x \implies y \sqsubseteq x \narrow y \sqsubseteq x$,
  and for every decreasing chain $x_0\sqsupseteq x_1\sqsupseteq x_2\sqsupseteq \ldots$
  the chain $y_0\sqsupseteq y_1\sqsupseteq y_2\sqsupseteq \ldots$, where $y_0=x_0$ and 
  $y_{i+1}=y_i\narrow x_{i+1}$, is not strictly decreasing.

The narrowing operator is classically used in a separate phase, starting with a variable 
assignment that satisfies all equations of the constraint system. For each variable $x_i$,
$x'_i=F_i(x_0,\ldots,x_{n-1})$ is calculated. Because $F_i$ is monotone, the values
$(x_0\narrow x_0',\ldots,x_{n-1}\narrow x_{n-1}')$ also satisfy all the equations of 
the constraint system. Such recomputation is done until stabilization, i.e., until the 
values stop decreasing, and this is guaranteed, by the definition of the narrowing operator,
to happen in finite number of steps. 

In the case of non-monotone functions $F_i$ and domains with infinitely ascending chains, 
we cannot use narrowing --- the newly computed value might be larger than the current value. 
This is, clearly, a problem if precision is crucial.
%
Therefore, we would like to have a \emph{simple} and \emph{robust} technique 
that works as well as the known solvers for functions with good properties 
and gives its best effort for functions with bad properties.
 





==> improved.tex <==
%!TEX root = main.tex
\section{Enhanced Technique}

Given a constraint system described by functions $F_i:L \to L$ and an operator $\Box:L \to L \to L$,
we say that $\vec y = (y_0,\ldots,y_n)$ is a $\Box$-solution, if for all $0\leq i<n$ we have 
$y_i = y_i\,\Box\,F_i\;\vec y$. 
%
Similarly, an algorithm is called a $\Box$-solver if given a constraint system provides 
an iteration strategy that produces a $\Box$-solution by sequentially applying 
the function $G^{\Box}$.




==> side-2.tex <==
\section{Perspective: Side-effecting systems of equations}\label{s:side}

Generic solving, as we have discussed in the preceding sections
cannot generally be extended to right-hand sides $f_x$ that
not only return a value for the left-hand side $x$ of the equation
$x= f_x$, but additionally may produce \emph{side effects}
to other variables as well. This extension which recasts \emph{assert}-statements
within {\sc Prolog} or {\sc Datalog} programs has been 
advocated in \cite{Apinis12} for an elegant treatment of
interprocedural analysis using partial contexts and 
flow-insensitive variables.

\begin{example}
\end{example}
%
In general, several side effects may occur to the
same variable $z$. Over an arbitrary domain of values, though,
it remains unclear how the multiple contributions
to $z$ should be combined. Therefore in this section,
we assume that the values of variables are taken from
a \emph{lattice} $\mathbb D$ and also that right-hand sides are
\emph{pure}. For side-effecting constraint systems this means
that evaluating a right-hand side $f_x$ applied to 
functions ${\sf get}:{\it Vars}\to{\mathbb D}$ and 
${\sf set}:{\it Vars}\to{\mathbb D}\to{\bf unit}$, 
consists of a sequence of variable lookups by means
of calls to the first argument function ${\sf get}$ 
and side effects to variables by means of calls to
the second argument function ${\sf set}$ which is
terminated by returning a contribution in $\mathbb D$
for the corresponding left-hand side.

%
Subsequently, we assume that each right-hand side $f_x$
produces no side effect to $x$ itself and also
to each variable $z\neq x$ at most one side effect.
Technically, the right-hand side $f_x$ of $x$ with side effects
can be considered as a succinct representation
of a function $\bar f_x$ that takes a variable assignment $\rho$
and does not return just a single value, but again
another variable assignment $\rho'$ where 
$\rho'(x)$ equals the return value computed by $f_x$ for $i{\sf get}=\rho$,
and for $z\neq x$, $\rho'(z) = d$ if during evaluation of $f_x\,{\sf get}\,{\sf set}$,
${\sf set}$ is called for $z$ and $d$. Otherwise, i.e., if no side effect occurs
to $z$, $\rho'(z)=\bot$.
%
A post solution of a system $x=f_x,x\in{\it Vars},$
of equations with side effects then is an assignment
$\rho:{\it Vars}\to{\mathbb D}$ such that for every
$x\in{\it Vars}$, $\rho\sqsupseteq \bar f_x\,\rho$.
%
A \emph{partial} post solution with domain ${\sf dom}\subseteq{\it Vars}$
is an assignment $\rho:{\sf dom}\to{\mathbb D}$ such that for every
$x\in{\sf dom}$, evaluation of $f_x$ for $\rho$ accesses only variables
in ${\sf dom}$ and also produces side effects only to variables in ${\sf dom}$.

In the following, we present a variant ${\bf SLR}^+$
of the algorithm {\bf SLR} from section \ref{s:local}
that for arbitrary such systems returns a partial post solution---whenever
it terminates. Moreover, the enhanced solver ${\bf SLR}^+$
is guaranteed to terminate whenever all right-hand sides $f_x$
are \emph{monotonic}, i.e., the functions $\bar f_x$ all are monotonic. 

Conceptually, the algorithm ${\bf SLR}^+$ creates for each side effect
to variable $z$ inside the right-hand side of $x$,
a fresh variable $\angl{x,z}$ which receives that
single value during evaluation of the right-hand side $f_x$.
%
Furthermore, the algorithm maintains for every variable $z$ an auxiliary set
${\sf set}\,z$ which consists of all variables $x$ whose right-hand sides
may possibly contribute to the value of $z$ by means of side effects.
%
Accordingly, the original system of side-effecting equations
is (implicitly) transformed in the following way:
\begin{enumerate}
\item	Inside a right-hand side $f_x$, the
	side effect ${\sf side}\,z\,d$ is implicitly replaced with
	\[
	{\sf side}\,\angl{x,z}\,d
	\]
	while additionally, $x$ is added to the set ${\sf set}\,z$.
\item	The new right-hand side for a variable $x$ then is extended
	with an evaluation of the variables in ${\sf set}\,x$.
\end{enumerate}
The $\upd$-operator is applied whenever a new contribution to 
one of the variables $\angl{x,z}$ occurs, and also whenever the 
return value of the new right-hand side for $x$ is combined with
the previous value of $x$. Let us now list the required modifications of the
algorithm {\bf SLR}. 

First, the function ${\sf init}\,y$ is extended with an extra initialization of 
the set ${\sf set}\,y$ with $\emptyset$, i.e., the line
\[
{\sf set}\,y\gets\emptyset
\]
is added to the body of ${\sf init}$.
%
The function ${\sf eval}$ remains literally unchanged.
%
Additionally, a function ${\sf side}$ is required for realizing
the side-effects during an evaluation of a right-hand side.
As the function ${\sf eval}$, also function ${\sf side}$ receives the left-hand side
of the equation under consideration as its first argument. We define:
\[
\begin{array}{lll}
{\sf side}\,x\,y\,d & = &
\begin{array}[t]{l}
{\bf if}\;(\angl{x,y}\not\in{\sf dom})\;\rho(\angl{x,y})\gets\bot;		\\
{\it tmp}\gets\rho(\angl{x,y})\upd d;		\\
{\bf if}\;({\it tmp}\neq\rho(\angl{x,y})\;\{	\\
\qquad\rho(\angl{x,y})\gets{\it tmp};		\\
\qquad{\bf if}\;(y\not\in{\sf dom})\;\{		\\
\qquad\qquad{\sf init}\,y;			\\
\qquad\qquad{\sf set}\,y\gets\{x\};			\\
\qquad\qquad{\sf solve}\;y;				\\
\qquad\}\;{\bf else}\;\{				\\
\qquad\qquad{\sf set}\,y\gets{\sf set}\,y\cup\{x\};			\\
\qquad\qquad{\it stable}\gets{\it stable}\setminus\{y\};		\\
\qquad\qquad{\sf add}\,Q\,y;		\\
\qquad\}				\\
\}						\\
\end{array}
\end{array}
\] 
When called with $x,y,d$, the function ${\sf side}$ is meant 
first to initialize the variable $\angl{x,y}$ if it is not yet contained
in ${\sf dom}$.
Then the new side effect $d$ is combined with the old value of $\angl{x,y}$
by means of the operator $\upd$.
If this combined value is different from the old value of $\rho$ for $\angl{x,y}$,
$\rho\,\angl{x,y}$ is updated. Subsequently, the set ${\sf set}\,y$ receives the
variable $x$, and the variable $y$ is triggered
for reevaluation. 
%
If $y$ has not yet been encountered, 
$y$ is initialized,
${\sf set}\,y$ is set to $\{x\}$, and then ${\sf solve}\,y$ is called immediately.
Otherwise,
$x$ is only added to ${\sf set}\,y$, and $y$ is scheduled for reevalutation
by destabilzing $y$ first and then inserting $y$ into the heap $Q$.
% i.e., side effect formerly realized from $x$ to $y$ 

the third modification concerns 
the procedure ${\sf solve}$.
There,
the call of the right-hand side $f_x$ now receives ${\sf side}\,x$
as a second argument and additionally evaluates all variables
collected in ${\sf set}\,x$. the corresponding new line reads:
\[
\begin{array}{l}
% {\sf solve}\,x\;= \\
% \qquad{\bf if}\;(x\not\in{\sf stable})\;\{      \\
% \qquad\qquad{\sf stable}\gets{\sf stable}\cup\{x\};     \\
% \qquad\qquad
{\bf if}\,(x\in{\sf Glob})\;{\it tmp}\gets\bigsqcup\{\rho\angl{z,x}\mid z\in{\sf set}\,x\};	\\
{\bf else}\; {\it tmp}\gets\rho(x)\;\upd\;
	(f_x\,({\sf eval}\,x)\;({\sf side}\,x);
% \qquad\qquad{\bf if}\;({\it tmp}\neq\rho(x))\;\{        \\
% \qquad\qquad\qquad\rho(x)\gets{\it tmp};        \\
% \qquad\qquad\qquad W\gets{\sf infl}(x); \\
% \qquad\qquad\qquad {\bf forall}\;(y\in W)\;{\sf add}\;Q\;y;     \\
% \qquad\qquad\qquad {\sf stable}\gets{\sf stable}\backslash W;   \\
% \qquad\qquad\qquad {\sf infl}(x)\gets\emptyset; \\
% \qquad\qquad\qquad {\bf while}\;(\neg({\sf empty}\,Q)\wedge{\sf min\_key}\,Q\leq {\sf key}\,x)\;\;\\
% \qquad\qquad\qquad\qquad        {\sf solve}\,({\sf extract\_min}\;Q);   \\
% \qquad\qquad\}                                                  \\
% \qquad\}
\end{array}
\]

Analogously to theorem \ref{t:local} from the last section, we obtain:

\begin{theorem}\label{t:side}
\begin{enumerate}
\item
When applied to any system of pure equations with side effects, the algorithm ${\bf SLR}^+$
returns a  post solution---whenever it terminates.
\item
Assume that ${\bf SLR}^+$ is
applied to a system of pure equations
over a complete lattice ${\mathbb D}$ where
each right-hand side is monotonic.
Then for any initial variable assignment $\rho_0$, ${\bf SLR}^+$
is guaranteed to terminate and thus always to return
a partial post solution---whenever only finitely many variables are encountered.
\end{enumerate}
\end{theorem}





==> single.tex <==
%!TEX root = main.tex
\section{Single iteration Widening/Narrowing}



\begin{lstlisting}[mathescape,morekeywords={begin}]
  x := ($\bot$, ..., $\bot$)
  y := $\bot$
  let rec solve i =
    if i $\geq$ 0 then {
      do {
        x$_i$ := y;
        solve (i-1);
        y := x$_i$ $\upd$F$_i$(x$_0$, $\ldots$,x$_n$)
      } while (x$_i\neq{}$y)
    }
\end{lstlisting}

==> topo.tex <==
\section{Box-based solvers and weak topological orderings}

In this section, we want to adapt the algorithms in \cite{ApinisSV13} with the
support for weak topological orderings instead of only variable priorities. 
First of all, we recall what is a weak topological orderings in our setting.

\begin{definition}[Hierarchical ordering \cite{Bourdoncle93}]
A \emph{hierarchical ordering} of a set $S$ is a well-parenthesized 
permutation of this set without two consecutive ``(''.
\end{definition}

In other words, a hierarchical ordering is a string over the alphabet
$S$ augmented with left and right parenthesis. The elements between two 
matching parentheses are called a \emph{component} and the first element of a 
component is called the  \emph{head}. The set  of heads of the 
components containing the element $l$ is denoted by $\omega(l)$. 

\begin{example}
\label{ex:ho}
Two hierarchical ordering for $S=\{1, \ldots, 10\}$ are $1 ~
2 ~ 3 ~ 4 ~ 5 ~ 6 ~ 7 ~ 8 ~ 9 ~ 10$ and $1 ~ (2 ~ 3 ~ 5 ~ (6 ~ 7 ~  9) ~ 8 ~ 
10) ~ 4$. In the second ordering, the heads are $2$ and $6$ and we have 
$\omega(4)=\emptyset$, $\omega(5)=\{2\}$ and $\omega(7)=\{2,7\}$.
\end{example}

A hierarchical ordering induces a total ordering, that we denote by $\preceq$, 
corresponding to the permutation of the elements. 

Now consider a set of data-flow equations. For each unknown $x$ we define 
$\dep_x$ according to \cite{ApinisSV13}.

\begin{definition}[Weak topological ordering \cite{Bourdoncle93}]
A \emph{weak topological ordering} of a system of data-flow equations is a 
hierarchical ordering of its unknowns such that, if $u \in \dep_v$
either $u \prec v$ or $v \preceq u$ and $v \in \omega(u)$. \footnote{In 
\cite{Bourdoncle93}, the first condition was $u \prec v \wedge v \notin 
\omega(u)$. However, the second conjunct is implied by the first one.}
\end{definition}

\begin{example}
\label{ex:wto}
Consider this system of data-flow equations:
\begin{align*}
x_1 &= [0,0] \times \Z\\
x_2 &= x_1 \vee x_{10}\\
x_3 &= x_2 \wedge ([-\infty,9] \times \Z)\\
x_4 &= x_2 \wedge ([10,\infty] \times \Z)\\
x_5 &= \mathit{first}(x_3) \times [0,0] \\
x_6 &= x_5 \vee x_9\\
x_7 &= x_6 \wedge (\Z \times [-\infty,9])\\
x_8 &= x_6 \wedge (\Z \times [10,\infty])\\
x_9 &= x_7 + ([0,0] \times [1,1])\\
x_{10} &= x_8 + ([1,1] \times [0,0])
\end{align*}
A possible w.t.o.~for such a system is: $x_1 ~ (x_2 ~ x_3 ~ x_5 ~ (x_6 ~ x_7 
~  x_9) ~ x_8 ~ x_{10}) ~ x_4$.
\end{example}

In the algorithms to come, we will need the following operators on
hierarchical orderings. 

\begin{definition}
Given a hierarchical ordering $\preceq$ for a set $S$, we define:
\begin{itemize}
\item $\head_\preceq(i)$ is true if $i$ is an head, i.e., if $i \in 
\omega(i)$, false  otherwise
\item $\nextinc_\preceq(i)$ is the next element of $i$ if there is no symbol 
$)$ between them, it is $\bot$ otherwise
\item $\textsf{next}_\preceq(i)$ is the next element of $i$ if it exists, $\bot$ 
otherwise
\item if $i$ precedes an head element $j$, $\skipc_\preceq(i)$, returns the 
element after the inner component which starts at $j$ and within the same 
component of $i$, if it exists.  It is $\bot$ otherwise.
\end{itemize}
We omit $\preceq$ from the subscripts of $\head$, $\nextinc$, $\textsf{next}$ and 
$\skipc$ when  it is clear from the context.
\end{definition}

\begin{example}
\label{ex:wto2}
On the w.t.o. given in Example~\ref{ex:wto}, we have $\textsf{next}(x_1)=x_2$, 
$\textsf{next}(x_{i})=x_{i+1}$ for each $i < 10$, $\textsf{next}(x_{10})=\bot$. Moreover, 
$\nextinc$ is defined as $\textsf{next}$, with the difference that $\nextinc(x_9)= 
\nextinc(x_{10})=\bot$. Finally $\skipc(x_1)=x_4$ and $\skipc(x_5)=x_8$.
\end{example}

\begin{example}
\label{ex:wto3}
For the h.o. $1 ~ 2 ~ (3 ~ (4 ~ 5)) ~ 6$ we have $\skipc(2)=6$ and 
$\skipc(3)=\bot$, since there is no element after $(4 ~ 5)$ which is  in the 
same component as $3$. 
\end{example}

\subsection{First algorithms}

We first define al algorithm which implements a recursive iteration strategy. 
The main idea of the recursive strategy is that inner components do stabilize 
before outer components. Figure~\ref{prg:rec} contains the source of the 
algorithm.

\begin{figure}
\centering
\begin{tabular}{c}
\begin{lstlisting}
void solve(i) {
  if (i==@$\bot$@) return
  if (not (head i)) {
    @$\rho(x_i) \leftarrow f_i \rho$@
    solve (next i)
  } else {
    @$\rho(x_i) \leftarrow \rho(x_i) \Box f_i \rho$@
    do {
      old @$\leftarrow \rho(x_i)$@
      solve (next i)
      @$\rho(x_i) \leftarrow \rho(x_i) \Box f_i \rho$@
    } while (@$\rho(x_i) \neq $@ old)
    solve (skip i)
  }
}
\end{lstlisting}
\end{tabular}
\caption{\label{prg:rec}The algorithm REC which performs a recursive iteration 
strategy.}
\end{figure}

Given a set of data-flow equations with unknowns $x_1, \ldots, 
x_n$, consider the w.t.o. $x_n ~ (x_{n-1} ( ~ \cdots (x_1 (x_0)) \cdots 
))$ where all parenthesis close at the end. Then $\head(i)$ is always true and 
$\skipc(i)$ is always $\bot$.  The order that data-flow equations are 
considered in  Algorithm 1 is almost the same order followed by the RR 
algorithm, with the difference 
that we always perform an update of $\rho(x_i)$ before solving for $x_{i-1}$.

